Juggernaut: Efficient Crypto-Agnostic Byzantine Agreement

It is well known that a trusted setup allows one to solve the Byzantine agreement problem in the presence of $t<n/2$ corruptions, bypassing the setup-free $t<n/3$ barrier. Alas, the overwhelming majority of protocols in the literature have the caveat that their security crucially hinges on the security of the cryptography and setup, to the point where if the cryptography is broken, even a single corrupted party can violate the security of the protocol. Thus these protocols provide higher corruption resilience ($n/2$ instead of $n/3$) for the price of increased assumptions. Is this trade-off necessary? We further the study of crypto-agnostic Byzantine agreement among $n$ parties that answers this question in the negative. Specifically, let $t_s$ and $t_i$ denote two parameters such that (1) $2t_i + t_s < n$, and (2) $t_i \leq t_s < n/2$. Crypto-agnostic Byzantine agreement ensures agreement among honest parties if (1) the adversary is computationally bounded and corrupts up to $t_s$ parties, or (2) the adversary is computationally unbounded and corrupts up to $t_i$ parties, and is moreover given all secrets of all parties established during the setup. We propose a compiler that transforms any pair of resilience-optimal Byzantine agreement protocols in the authenticated and information-theoretic setting into one that is crypto-agnostic. Our compiler has several attractive qualities, including using only $O(\lambda n^2)$ bits over the two underlying Byzantine agreement protocols, and preserving round and communication complexity in the authenticated setting. In particular, our results improve the state-of-the-art in bit complexity by at least two factors of $n$ and provide either early stopping (deterministic) or expected constant round complexity (randomized). We therefore provide fallback security for authenticated Byzantine agreement for free for $t_i \leq n/4$.

==> cons_validity.tex <==
\section{Asynchronous Validity-Extended Graded Consensus}\label{sec:gcmvb}
%\todo[inline]{Note that we assume that at most one message per 'type' is accepted in MV and GC (which is trivial to implement) (otherwise e.g. step 4 of GC would lead to $O(n^3)$ complexity; I think security is also violated without this)}
We introduce two primitives that are weaker than consensus and thus do not require additional assumptions in asynchrony to solve (ie. coin flipping).
Looking forward, neither primitive guarantees termination itself but will terminate when used in our Byzantine agreement protocol.
We note that for our MV-broadcast and graded consensus protocols in this section we assume that at most one message per `type' is accepted by a party (which is trivial to implement).
This step is taken in order to ensure security of the protocols and bound their communication complexity. 

\subsection{MV-Broadcast}
The first primitive is MV-broadcast which was defined in \cite{mostefaoui2017signature} for the asynchronous setting.
The goal of MV-broadcast is to `filter' messages for consensus: parties input a value $v$ and output a set $S$ such that each value inside was either MV-broadcasted by an honest party (validity 1) or is a default value.
It guarantees a limited form of agreement on values (validity 2 and inclusion).
For MV-broadcast, we consider default value $\bot_{mv} \not\in V$.

\begin{definition}[Multivalued broadcast (MV-broadcast)~\cite{mostefaoui2017signature}]
Let $\Pi$ be a protocol executed by parties $P_1, \dots, P_n$, where each party $P_i$ begins holding input $v_i \in V$.
\begin{itemize}
\item \emph{\textbf{Validity 1:}} $\Pi$ achieves $t$-$\mathsf{validity}$ $\mathsf{1}$ if whenever at most $t$ parties are corrupted, if an honest party outputs a set $S$ such that $v \in S$ and $v \neq \bot_{mv}$, then $v$ was input by an honest party.
\item \emph{\textbf{Validity 2:}} $\Pi$ achieves $t$-$\mathsf{validity}$ $\mathsf{2}$ if the following holds whenever at most $t$ parties are corrupted: if every honest party's input is equal to the same value $v$, then no honest party outputs a set containing $\bot_{mv}$.
\item \emph{\textbf{Inclusion:}} $\Pi$ achieves $t$-$\mathsf{inclusion}$ if the following holds whenever at most $t$ parties are corrupted: if honest $P_i$ and $P_j$ output sets $S_i$ and $S_j$ respectively, then $S_i = \{w\} \Rightarrow w \in S_j$ (note $w = \bot_{mv}$ is possible).
\item \emph{\textbf{Liveness:}} $\Pi$ achieves $t$-$\mathsf{liveness}$ if whenever at most $t$ parties are corrupted, every honest party outputs a set $S$ where each $v \in S$ is such that $v \in V \cup \{\bot_{mv}\}$.
\item \emph{\textbf{Validity with liveness:}} $\Pi$ achieves $t$-$\mathsf{validity}$ $\mathsf{with}$ $\mathsf{liveness}$ if the following holds whenever at most $t$ parties are corrupted: if every honest party's input is equal to the same value $v$, every honest party outputs the set $S = \{v\}$.
\end{itemize}
\end{definition}
In \cite{mostefaoui2017signature}, validity 1 and validity 2 are denoted as justification and obligation, respectively.
We additionally define validity with liveness which our protocol will satisfy with $t_s$ corruptions in synchrony.
We present our MV-broadcast construction in Figure~\ref{fig:mvbroadcast}.

\iffalse
MV-broadcast, or multivalued broadcast, (not to be confused with \textit{secure broadcast} or \textit{broadcast}) was introduced in \cite{mostefaoui2017signature} as a building block to construct intrusion-tolerant consensus.
Eventually, $P_i$ outputs a non-empty set which contains one or more of either a \textit{validated} value or a default value denoted as $\bot_{mv}$.
This default value, however, cannot be MV-broadcast by a party.
A validated value is one that must have been MV-broadcast by at least one honest party.
\fi

\begin{figure}[ht!] 
\centering
\fbox{
\parbox{0.95\textwidth}{
\centering $\Pi_{\MV}^{t_a, t_s}(v_i)$
\begin{enumerate}
\item Set $\output = \ready = \false$ and $M_2(v) = \emptyset$ for all $v \in V$.
\item For every $v \in V$, let $M_1(v)$ be the (initially empty) set of parties from which $P_i$ has received $(\mvi, v)$.
\item Multicast $(\mvi, v_i)$.
\item Upon receiving $(\mvi, v)$ messages on the same value $v$ (possibly $\bot_{mv}$) from $n - t_s$ distinct parties: if $\ready = \false$, set $\ready = \true$ and multicast $(\mvii, v)$.
\item Upon receiving $(\mvi, v)$ messages on the same value $v$ from $t_s + 1$ distinct parties: if $(\mvi, v)$ not yet multicast, multicast $(\mvi, v)$.
\item Upon receiving $(\mvi, v_{max})$ for $v_{max}$ such that $v_{max} = \arg\max_{v' \in V}|M_1(v')|$: if $|\cup_{v' \in V}M_1(v')| - |M_1(v_{max})| \geq t_s + 1$ and $(\mvi, \bot_{mv})$ not yet multicast, multicast $(\mvi, \bot_{mv})$.
\item Upon having $|\cup_{v\in V} M_2(v)| \geq n-t_s$: if $\output = \false$, set $\output = \true$ and output $\{v : |M_2(v)| > 0\}$.
\end{enumerate}
Updating $M_2(v)$:
\begin{itemize}
\item[(i)] Upon receiving $(\mvii, v)$ from $P_j$: if previously received messages $(\mvi, v)$ on the same value from $n - t_s$ distinct parties, set $M_2(v) = M_2(v) \cup \{j\}$.
\item[(ii)] Upon receiving $(\mvi, v)$ messages on the same value $v$ from $n - t_s$ distinct parties: set $M_2(v) = M_2(v) \cup \{j : P_j$ previously sent $(\mvii, v)\}$.
\end{itemize}
}
}
\caption{MV-broadcast from the perspective of party $P_i$.}
\label{fig:mvbroadcast}
\end{figure}

$\Pi_{\MV}^{t_a, t_s}$ works as follows.
Consider honest $P_i$ with input value $v_i\in V$.
For each $v\in V$, $P_i$ manages tracks two local initially empty sets $M_1(v)$ and $M_2(v)$.
There are two types of messages multicast by $P_i$, $(\mvi,v)$ and $(\mvii,v)$ for $v \in V$.
The distinction between $\mvi$ and $\mvii$ is simply to multicast $(\mvii, v)$ as soon as enough $(\mvi,v)$ messages (on the same value $v$) were received, which is tracked via the set $M_1(v)$.
By definition, $M_1(v)$ is the set of parties from which $P_i$ has received a $(\mvi,v)$ message.
On the other hand, $M_2(v)$ keeps track of whether value $v$ is validated (was input by an honest party) or not. 

After variable initialisation, $P_i$ multicasts $(\mvi, v_i)$ (step 3).
For a given $v$, on first receipt of $(\mvi, v)$ from $t_s + 1$ parties, $P_i$ multicasts it (step 5).
On first receipt of $(\mvi, v)$ from $n - t_s$ parties for \textit{any} $v$ (step 4), $P_i$ sets $\ready = \true$ and multicasts $(\mvii, v)$ i.e. $P_i$ champions $v$ for output.
At this time, $M_2(v)$ is also updated (step (i)),
If too many values were received, i.e. $|\cup_{v' \in V}M_1(v')| - |M_1(v_{max})| \geq t_s + 1$ where $v_{max} = \arg\max_{v' \in V}|M_1(v')|$, then $P_i$ signals this by multicasting $(\mvi, \bot_{mv})$ (step 6).
At any time, $P_i$ updates the set $M_2(v)$ as $M_2(v) = M_2(v) \cup \{j\}$ after it receives 
proposal $(\mvii,v)$ by party $P_j$ whenever $P_i$ has received the message $(\mvi,v)$ from $\geq n-t_s$ distinct parties.
Finally, when $P_i$ first receives $n-t_s$ $(\mvii,w)$ messages where $n - t_s$ $(\mvi, w)$ messages were also received (on possibly different values $w$), captured by the predicate $|\cup_{v\in V} M_2(v)| \geq n-t_s$ in step 7, $P_i$ outputs $\{v : |M_2(v)| > 0\}$. \\

\noindent \textbf{Communication Complexity.} We argue in the following that the communication complexity of our MV-broadcast protocol $\Pi_{\MV}$ is bounded by $O(n^3)$. Having a look at Figure \ref{fig:mvbroadcast}, we see that every honest party multicasts at most one message of the form $(\mvii,-)$ (line 4). Furthermore, a message of the form $(\mvi,v)$ for some $v\neq \bot_{mv}$ is multicast if it was received from at least $t_s+1$ distinct parties, ensuring that the message had to come from at least one honest party (line 5). In particular, an honest party only $\mvi$-multicasts at most $n-t_s$ times. Moreover, every honest party multicasts at most one message of the form $(\mvi, \bot_{mv})$ (line 6).  As a result, the overall communication complexity of $\Pi_{\MV}$ is bounded by $O(n^3)$.

\begin{theorem}
	Let $n,t_s,t_a$ be such that $0 \le t_a < \frac{n}{3} \le t_s < \frac{n}{2}$ and $t_a + 2 \cdot t_s < n$.
	Then MV-broadcast protocol $\Pi_{\MV}^{t_a, t_s}$ (Figure~\ref{fig:mvbroadcast}) satisfies $t_s$-validity 1, $t_s$-validity 2, $t_s$-valid with liveness, $t_a$-inclusion and $t_a$-liveness.
\end{theorem}

\noindent We prove this by proving the following lemmas.
\input{mvproof.tex}

\subsection{Graded Consensus}
\daniel{this has 3 grades}
Next, we define our graded consensus primitive.
In graded consensus, each party inputs a value but outputs both a value $v \in V \cup \{\bot\}$ and a corresponding grade $g \in \{0, 1, 2\}$.
\textit{Binary} graded consensus (i.e., where $V = \{0, 1\}$) was previously considered for building network-agnostic binary agreement in \cite{TCC:BluKatLos19}.
Our primitive will also require an intrusion tolerance property that we define below.

\begin{definition}[Graded consensus]
Let $\Pi$ be a protocol executed by parties $P_1, \dots, P_n$, where each party $P_i$ begins holding input $v_i \in V$.
\begin{itemize}
\item \emph{\textbf{Graded validity:}} $\Pi$ achieves $t$-$\mathsf{graded}$ $\mathsf{validity}$ if the following holds whenever at most $t$ parties are corrupted: if every honest party's input is equal to the same value $v$, then all honest parties output $(v, 2)$.
\item \emph{\textbf{Graded consistency:}} $\Pi$ achieves $t$-$\mathsf{graded}$ $\mathsf{consistency}$ if the following holds whenever at most $t$ parties are corrupted: (1) If two honest parties output grades $g, g'$, then $|g - g'| \leq 1$. (2) If two honest parties output $(v, g)$ and $(v', g')$ with $g, g' \geq 1$, then $v = v'$.
\item \emph{\textbf{Liveness:}} $\Pi$ achieves $t$-$\mathsf{liveness}$ if whenever at most $t$ parties are corrupted, every honest party outputs $(v, g)$ with either $v \in V$ and $g \geq 1$, or $v = \bot$ and $g = 0$.
\item \emph{\textbf{Intrusion tolerance:}} $\Pi$ achieves $t$-$\mathsf{intrusion}$ $\mathsf{tolerance}$ if whenever at most $t$ parties are corrupted, if $(v, g)$ is output by an honest party and $g \geq 1$, then $v$ was input by an honest party.
\end{itemize}
%If $\Pi$ achieves $t$-graded validity, $t$-graded consistency and $t$-liveness, we say it is $t$-$\mathsf{secure}$. 
\end{definition}

%In graded consensus, each party outputs a value $v \in V \cup \{\bot\}$ alongside a grade $g\in \{0,1,2\}$.
We construct a multivalued graded consensus protocol $\Pi_{\GC}^{t_a, t_s}$ (Figure~\ref{fig:mvgc})
Our protocol requires two (implicitly domain separated) instances of $\Pi_{\MV}^{t_a, t_s}$ which we denote by $\MV_1$ and $\MV_2$ with default values $\bot_{mv1}$ and $\bot_{mv2}$ respectively.

\begin{figure}[ht!]
\centering
\fbox{
\parbox{0.95\textwidth}{
\centering $\Pi_{\GC}^{t_a, t_s}(v_i)$
\begin{itemize}
	\item[1.] Set $\output = \false, \val = \bot, \aux = \bot$.
	\item[2.] For every $v\in V$, let $R(v)$ be the set of parties from which $P_i$ has received $(\msg, v)$ for $\msg \in \{\init, \echo\}$. Initially, set $R(v) = \emptyset$ for all $v\in V$. 
	\item[3.] Multicast the message $(\init, v_i)$.
	\item[4.] Upon receiving $(\init, v)$ messages on the same value $v$ from $t_s + 1$ distinct parties: if $v \neq v_i$ and $(\echo, v)$ not yet multicast, multicast $(\echo, v)$.
	\item[5.] Upon receiving $(\msg, v)$ for some $\msg \in \{\init, \echo\}$ and $v$ when $\output = \false$:
	\begin{itemize}
	\item[(a)] If $v \neq v_i$ and $|R(v)| \geq t_s + 1$, set $\output = \true$ and $\val = \bot_{rd}$.
	\item[(b)] If $|R(v)| \geq n - t_s$, set $\output = \true$ and $\val = v$.
	\item[(c)] If $|\cup_{v' \in V} R(v')| - m \geq t_s + 1$ for $m = \max_{v' \in V}|R(v')|$, set $\output = \true$ and $\val = \bot_{rd}$.
	\item[(d)] If $\output = \true$, run $\MV_1$ using input $\val$.
	\end{itemize}
	\item[6.] Upon receiving output $S_1$ from $\MV_1$: if $S_1 = \{v\}$, set $\aux = v$. Run $\MV_2$ using input $\aux$.
	\item[7.] Upon receiving output $S_2$ from $\MV_2$:
\begin{itemize} 
\item[(a)] If $S_2 = \{v\}$ and $v \not\in \{\bot_{rd}, \bot_{mv1}, \bot_{mv2}, \bot\}$, output $(v, 2)$.
\item[(b)] Otherwise, if $\exists \ v \in S_2$ s.t. $v \not\in \{\bot_{rd}, \bot_{mv1}, \bot_{mv2}, \bot\}$, output $(v, 1)$.
\item[(c)] Otherwise, output $(\bot, 0)$.
\end{itemize}
		\end{itemize} 
}
}
\caption{Multivalued graded consensus from the perspective of party $P_i$.}
\label{fig:mvgc}
\end{figure}

$\Pi_{\GC}^{t_a, t_s}$ works as follows.
Suppose (honest) $P_i$ inputs $v_i$.
In addition to messages from MV-broadcast, $\Pi_{\GC}$ uses two message types, namely $(\init,v)$ and $(\echo,v)$ for some $v \in V$.
After initialising variables, $P_i$ multicasts $(\init, v_i)$ (and doesn't send $\init$ messages hereafter).
On receipt of messages $(\msg, v)$ (where $\msg \in \{\init,\echo\}$ from $t_s + 1$ parties (and thus an honest party input $v$), $P_i$ multicasts $(\echo, v)$ if not yet done.
Except for these steps, communication takes place through $\MV_1$ and $\MV_2$.

Let $R(v)$ be the set of parties from which $P_i$ has received a message of the form $(\init, v)$ or $(\echo,v)$ (step 2).
Then, whenever $P_i$ receives a message $(\msg, v)$, $P_i$ checks some conditions to determine whether it can input a value to $\MV_1$ (after which the conditions are ignored).
If $|R(v)| \geq t_s + 1$ and $v \neq v_i$, $P_i$ inputs $\bot_{rd}$ to $\MV_1$, indicating disagreement between two honest parties.
Similarly, if $|\cup_{v' \in V} R(v')| - \max_{v' \in V}|R(v')| \geq t_s + 1$, $P_i$ inputs $\bot_{rd}$ to $\MV_1$.
If $|R(v)| \geq n - t_s$, indicating enough parties received $v$, $P_i$ inputs $v$ to $\MV_1$.

Then, $P_i$ eventually outputs a set $S_1$ from $\MV_1$.
If $|S| = \{v\}$, $P_i$ runs $\MV_2$ with that input; otherwise $P_i$ runs $\MV_2$ on input $\bot$ (step 6).
On outputting $S_2$ from $\MV_2$ (step 2), if $S_2 = \{v\}$ and not a default value, then it outputs $(v, 2)$.
Otherwise, if $S_2$ contains a non-default value, $P_i$ outputs that value and $g = 1$; else, $P_i$ outputs $(\bot, 0)$. \\

\noindent \textbf{Communication Complexity.} We argue in Lemma~\ref{lem:gccommunicationcomplexity} that the communication complexity of our graded consensus protocol $\Pi_{\GC}^{t_a, t_s}$ is bounded by $O(n^3)$. Furthermore, we argue that if the network happens to be asynchronous, then the communication complexity of the protocol improves to $O(n^2)$. On the other hand, if the networks happens to be synchronous and parties input the same values to the graded consensus protocol, then the communication complexity can trivially be bounded by $O(n^2)$. We elaborate more on these facts in Lemma~\ref{lem:gccommunicationcomplexity}.

\begin{theorem}
	Let $n,t_s,t_a$ be such that $0 \le t_a < \frac{n}{3} \le t_s < \frac{n}{2}$ and $t_a + 2 \cdot t_s < n$.
	Then graded consensus protocol $\Pi_{\GC}^{t_a, t_s}$ (Figure~\ref{fig:mvgc}) satisfies $t_s$-graded validity, $t_s$-intrusion tolerance, $t_a$-graded consistency and $t_a$-liveness.
\end{theorem}

\noindent We prove this by proving the following lemmas.

\input{gcproof.tex}


==> gc_jovan.tex <==
\section{Graded Consensus 1}

\begin{figure}[ht!] 
\centering
\fbox{
\parbox{0.95\textwidth}{
\centering $\Pi_{\GCone}(v_i)$\\
\textbf{Initialization: $\mathit{val}_i \gets v_i$}
\begin{itemize}

\item Round 1: Multicast $\mathsf{init}(v)$.

\item Round 2: If there exists $v \in \mathcal{V}$ such that at least $n - t_i$ $\mathsf{init}(v)$ messages are received, then perform the following steps: (1) use threshold signatures to create an $(n - t_i)$-certificate $\mathcal{C}(v)$ for $\mathsf{init}(v)$, (2) multicast $\mathcal{C}(v)$, and (3) decide $(v, 1)$.

\item Round 3: If (1) there exists $v \in \mathcal{V}$ such that $\mathcal{C}(v)$ is received, and (2) there does not exist $v' \neq v$ such that $\mathcal{C}(v')$ is received, then $\mathit{val}_i \gets v$.

\item Round 4: Let $(v^*, g^*) \gets \mathcal{GC}(\mathit{val}_i)$.
If not previously decided, decide $(v^*, g^*)$.

\end{itemize}

}
}
\caption{Authenticated $t_s$-secure and $t_i$-valid with termination $\GCone$}
\label{fig:gc_1_jovan}
\end{figure}

\paragraph{Validity in the signature-free world.}
First, we prove that $\Pi_{\GCone}$ satisfies validity in the signature-free world.

\begin{lemma} \label{lemma:init_correct_proposal}
If any correct process receives $n - t_i$ $\mathsf{init}(v)$ messages, then $v$ is the proposal of a correct process.
\end{lemma}
\begin{proof}
As $n > t_s + 2t_i$, we have that $n - t_i > t_i$.
Therefore, the lemma holds.
\end{proof}

\begin{theorem}
$\Pi_{\GCone}$ satisfies validity in the signature-free world.
\end{theorem}
\begin{proof}
Suppose all correct processes propose the same value $v \in \mathcal{V}$.
As there are at least $n - t_i$ correct processes and they all propose value $v$, every correct process eventually receives $n - t_i$ values for $v$ (and, by Lemma~\ref{lemma:init_correct_proposal}, only $v$).
Therefore, every correct process decides $(v, 1)$, thus concluding the proof.
\end{proof}

\paragraph{Validity in the signature world.}
We now prove that $\Pi_{\GCone}$ satisfies validity in the signature world.
Throughout the rest of the proof of the validity property, we suppose that all correct processes propose the same value $v$.

\begin{lemma} \label{lemma:validity_certificate}
If any $(n - t_i)$-certificate $\mathcal{C}(v')$ is formed, then $v' = v$.
\end{lemma}
\begin{proof}
As $\mathcal{C}(v')$ is formed and $n - t_i > t_s$ (given that $n > t_s + 2t_i$), there exists a correct process that sends an $\mathsf{init}(v')$ message for its proposal $v'$.
Given that all correct processes propose $v$, $v' = v$.
\end{proof}

\begin{lemma} \label{lemma:validity_round_2}
If any correct process decides some value $v'$ in round 2, then $v' = v$.
\end{lemma}
\begin{proof}
Let $p_i$ denote any correct process that decides some value $v'$ in round 2.
Therefore, $p_i$ receives an $\mathsf{init}(v')$ message for $v'$ from a correct process as $n - t_i > t_s$ (recall that $n > t_s + 2t_i$).
As all correct processes propose $v$, $v' = v$ and the lemma holds.
\end{proof}

\begin{theorem}
$\Pi_{\GCone}$ satisfies validity in the signature world.
\end{theorem}
\begin{proof}
Consider any correct process $p_i$ that decides; let $p_i$ decide $(v', g')$.
We distinguish two cases:
\begin{itemize}
    \item Let process $p_i$ decide in round $2$.
    In this case, $v' = v$ (due to Lemma~\ref{lemma:validity_round_2}) and $g' = 1$.
    Therefore, the statement of the theorem holds in this case.

    \item Let process $p_i$ decide in round (i.e., step) $4$.
    Here, every correct process that proposes to $\mathcal{GC}$ does so with value $v$.
    Indeed, if any correct process $p_j$ updates its $\mathit{val}_j$ variable in round $3$, Lemma~\ref{lemma:validity_certificate} proves that $\mathit{val}_j$ holds value $v$.
    Hence, the validity property of $\mathcal{GC}$ ensures that $v' = v$ and $g' = 1$.
\end{itemize}
As the statement of the theorem holds in both possible scenarios, the proof is concluded.
\end{proof}

\paragraph{Consistency in the signature world.}

\begin{lemma} \label{lemma:consistency_no_two_certificates}
No two $(n - t_i)$-certificates $\mathcal{C}(v)$ and $\mathcal{C}(v' \neq v)$ can be formed. 
\end{lemma}
\begin{proof}
By contradiction, suppose two certificates $\mathcal{C}(v)$ and $\mathcal{C}(v' \neq v)$ are formed.
Therefore, there are $n - t_i + n - t_i - n = n - 2t_i$ processes that participated in forming both certificates.
As $n > t_s + 2t_i$, $n - 2t_i > t_s$, which further implies that there is at least one correct process that participated in forming both certificates.
As this is impossible, we reach a contradiction.
\end{proof}

\begin{lemma} \label{lemma:consistency_round_2}
If any correct process decides $(v, 1)$ in round $2$, then all correct processes decide $(v, 1)$.
\end{lemma}
\begin{proof}
First, all correct processes that decide in round $2$ do decide $(v, 1)$ (due to Lemma~\ref{lemma:consistency_no_two_certificates}).
Moreover, every correct process $p_i$ sets its $\mathit{val}_i$ variable to $v$ in round $3$ (due to Lemma~\ref{lemma:consistency_no_two_certificates}).
Therefore, the validity property of $\mathcal{GC}$ ensures that all correct processes that decide in round (i.e., step) $4$ decide $(v, 1)$.
\end{proof}

\begin{theorem}
$\Pi_{\GCone}$ satisfies consistency.
\end{theorem}
\begin{proof}
To prove the theorem, we consider two possible scenarios:
\begin{itemize}
    \item Let there exist a correct process that decides $(v, 1)$ in round $2$.
    In this case, all correct processes decide $(v, 1)$ (by Lemma~\ref{lemma:consistency_round_2}).

    \item No correct process decides in round $2$.
    In this case, the consistency property follows directly from the consistency property of $\mathcal{GC}$.
\end{itemize}
As the statement of the theorem holds in both possible cases, the proof is concluded.
\end{proof}

==> gcproof.tex <==
\begin{lemma} \label{lem:gcgradedvalidity}
Let $t_s < n/2$. Then $\Pi_{\GC}^{t_a, t_s}$ achieves $t_s$-graded validity.
\end{lemma}
\begin{proof}
In order to prove $t_s$-graded validity, we show that  if every honest party’s input is equal to the same value $v$, then all honest parties output $(v, 2)$.
Let every honest party multicast $(\init, v)$ (line 3, Figure \ref{fig:mvgc}).
Since there are at most $t_s < t_s+1$ dishonest parties, no honest party echoes a value different from $v$ (line 4).
Therefore, from the perspective of every honest party $P_i$ the set $R(w)$ is of size $\le t_s$ for every $w\neq v$. In particular, conditions (a) and (c) of line 5 are not satisfied for the value $v$.
On the other hand, since there are at least $n-t_s$ honest parties that multicast $(\init,v)$, it is $|R(v)|\geq n-t_s$, and $P_i$ sets $\output = \true$ and $\val = v$ (line 5, condition (b)).
As this applies to every honest party, each of them run $\MV_1$ on the same input $v$ (line 5 (d)).
Now, $t_s$-validity with liveness from $\MV_1$ ensures that every honest party outputs the set $S_1 = \{v\}$.
As a result, each of them sets $\aux = v$ and runs $\MV_2$ again on input $v$ (line 6).
The same argument yields that every honest party outputs the set $S_2 = \{v\}$. Finally, as $v \notin \{\bot_{rd}, \bot_{mv1}, \bot_{mv2}, \bot\}$, every honest party outputs $(v,2)$ (line 7 (a)).
\qed
\end{proof}

\begin{lemma} \label{lem:gcgradedconsistency}
Let $t_a \leq t_s$ and $t_a + 2 \cdot t_s < n$. Then $\Pi_{\GC}^{t_a, t_s}$ achieves $t_a$-graded consistency.
\end{lemma}
\begin{proof}
In order to prove $t_a$-graded consistency, we show that (1) if two honest parties output grades $g,g'$, then $|g-g'|\le 1$, and (2) if two honest parties output $(v, g)$ and $(v',g')$ with $g, g' \geq 1$, then $v = v'$.

For the first clause, assume that there are two honest parties $P_i$ and $P_j$ where $P_i$ outputs $(v,2)$.
This means $P_i$'s output $S_2$ from $\MV_2$ is $S_2 = \{v\}$ with $v \notin \{\bot_{rd}, \bot_{mv1}, \bot_{mv2}, \bot\}$ (line 7 (a), Figure \ref{fig:mvgc}).
By $t_a$-inclusion of $\MV_2$, every honest party $P_j$ outputs a set $S_2$ such that $v\in S_2$ and therefore cannot output grade $g' = 0$ for its final decision (line 7 (c)).
This proves the first clause.

For the second clause, consider two honest parties $P_i$ and $P_j$ that output $(v,g)$ and $(v',g')$ respectively with $g, g' \geq 1$.
We write $S_2(P_k)$ for the output set $S_2$ from $\MV_2$ of party $P_k$; for the output set $S_1$ we likewise define $S_1(P_k)$.
In particular, $v\in S_2(P_i)$ and $v'\in S_2(P_j)$ with $v,v'\notin \{\bot_{rd}, \bot_{mv1}, \bot_{mv2}, \bot\}$ (line 7 (a) and (b)).
By $t_a$-inclusion of $\MV_2$, it follows that $v\in S_2(P_j)$ and thus $\{v,v'\}\subseteq S_2(P_j)$.
By $t_s$-validity 1 of $\MV_2$, $v'$ was input by some honest party $P_k$ to $\MV_2$.
In particular, $\aux=v'$ for party $P_k$ and thus $S_1(P_k) = \{v'\}$ (line 6).
Analogously, there is some honest party $P_l$ that input $v$ to $\MV_2$ and hence $S_1(P_l) = \{v\}$.
But by $t_a$-inclusion of $\MV_1$, it follows that $v = v'$, which concludes the proof.
\qed
\end{proof}

\begin{lemma} \label{lem:gcliveness}
Let $t_a \leq t_s$ and $t_a + 2 \cdot t_s < n$. Then $\Pi_{\GC}^{t_a, t_s}$ achieves $t_a$-liveness.
\end{lemma}
\begin{proof} 
In order to prove $t_a$-liveness, we show that every honest party outputs $(v,g)$ with either $v\in V$ and $g \geq 1$, or $v = \bot$ and $g = 0$ (line 7, Figure \ref{fig:mvgc}).
We consider the following predicate $P$: There is a value $v\in V$ such that after some finite time at least $t_s+1$ honest parties have multicast $(\init,v)$.
Consider the following two cases.
\begin{itemize} 
\item[(i)] The predicate $P$ is satisfied.
It follows that every honest party eventually multicasts $(\echo,v)$ (if not yet multicast $(\init,v)$) (line 4).
As there are at least $n-t_a \geq n-t_s$ honest parties, the predicate $|R(v)|\geq n-t_s$ in line 5 (b) becomes eventually true for every honest party and each of them sets $\output = \true$ and runs $\MV_1$ (line 5 (d)).
By $t_a$-liveness of $\MV_1$, every honest party outputs some set $S_1$ and runs $\MV_2$ on input $\aux$ (line 6).
And by $t_a$-liveness of $\MV_2$, every honest party outputs some set $S_2$ and finally outputs some graded value $(v,g)$ (line 7).
The requirement [$v\in V$ and $g \geq 1$, or $v = \bot$ and $g = 0$] is trivially satisfied by construction of $\Pi_{\GC}^{t_a, t_s}$ in its final step (line 7). 
\item[(ii)] The predicate $P$ is not satisfied.
This means there is no value $v$ that is multicast $(\init,v)$ by at least $t_s+1$ honest parties.
We consider an honest party $P_i$.
Let $v_{max}$ be its most often received value from distinct parties as defined in line 5 (c) and let $r$ be the number of honest parties that multicast $(\init,v_{max})$.
By assumption, we have $r \le t_s$.
Let $k\in [0,t_a]$ be the number of distinct dishonest parties from which $P_i$ has received the message $(\init,v_{max})$.
Clearly, at most $t_s+k \geq r+k$ distinct parties have sent the value $v_{max}$ to $P_i$.
Now assume that the waiting predicates [$|R(v)| \geq n - t_s$] and [for $w \neq v_i$ and $|R(w)| \geq t_s + 1$] in line 5 (a) and (b) are never satisfied (otherwise $P_i$ sets $\output = \true$ and proceeds with the execution of $\MV_1$).
Since $P_i$ does not terminate at these predicates, it receives a message from each honest party, that is from at least $n-t_a$ parties.
Hence, $P_i$ receives messages from at least $n-t_a+k$ distinct parties.
As a consequence, at least $(n-t_a+k)-(t_s+k) = n-t_a-t_s > t_s$ distinct parties have sent values different from $v$ to $P_i$.
As a result, the predicate $|\cup_{v' \in V} R(v')| - |R(v_{max})| \geq t_s + 1$ in line 5 (c) is eventually satisfied and $P_i$ runs $\MV_1$ on input $\val = \bot_{rd}$.
Therefore, every honest party runs $\MV_1$ on some input (line 5 (d)) and the remainder of the proof proceeds as in the previous case.
\end{itemize} 
\qed
\end{proof}

\begin{lemma} \label{lem:gcintrusiontolerance}
Let $t_s < n/2$. Then $\Pi_{\GC}^{t_a, t_s}$ achieves $t_s$-intrusion tolerance.
\end{lemma}
\begin{proof} 
In order to prove $t_s$-intrusion tolerance, we show that no honest party $P_i$ outputs a graded value $(v,g)$ with $g\geq 1$ that was multicast $(\init,v)$ by dishonest parties only.
For this, let there be $t_s$ dishonest parties that multicast $(\init,v)$ such that $(\init,v)$ is not multicast by any honest party.
Since $t_s+1 > t_s$, no honest party echoes $(\echo,v)$ the value $v$ and thus $v$ can be received only from the $t_s$ dishonest parties (line 4, Figure \ref{fig:mvgc}).
As a consequence, for every honest party $P_i$ it is $|R(v)| \le t_s < n-t_s$ and thus no honest party sets $\val$ equal to $v$ (line 5 (b)).
The claim follows from $t_s$-validity 1 of $\MV_1$ and $\MV_2$.
\qed
\end{proof}

\iffalse
\begin{theorem}
Let $t_a \leq t_s$ and $t_a + 2 \cdot t_s < n$. Then $\Pi_{\GC}^{t_a, t_s}$ is $t_a$-secure, $t_s$-intrusion tolerant and achieves $t_s$-graded validity.
\end{theorem}
\begin{proof}
This is clear from the above lemmata. Lemmata \ref{lem:gcgradedvalidity}, \ref{lem:gcgradedconsistency}, \ref{lem:gcliveness}, and \ref{lem:gcintrusiontolerance} give $t_a$-security, since $t_a \le t_s$. Also, Lemma \ref{lem:gcintrusiontolerance} gives $t_s$-intrusion tolerance and Lemma \ref{lem:gcgradedvalidity} gives $t_s$-graded validity.
\qed
\end{proof}
\fi

\noindent Finally, we bound the complexity of the protocol.
\begin{lemma} \label{lem:gccommunicationcomplexity}
Let $t_s < n/2$. The total communication complexity of the graded consensus protocol $\Pi_{\GC}^{t_a, t_s}$ is bounded by $O(n^3)$. Furthermore, if the underlying network is asynchronous, this improves to a communication complexity of $O(n^2)$. 
\end{lemma}
\begin{proof}
First, we show that each honest party may echo at most two messages $(\echo,-)$ with different values. For this, let $n = 2t_s+t_a+1 < 3(t_s+1)$ and consider an honest party $P_i$. Clearly, $P_i$ receives at most one message $(\init,-)$ from any other party, as it otherwise would know that the sender is dishonest. In order to multicast message $(\echo,v)$ for some $v\neq v_i$, $P_i$ needs to receive $(\init,v)$ from $t_s+1$ distinct parties (line 4, Figure \ref{fig:mvgc}). Since $n < 3(t_s+1)$, it follows that $P_i$ can echo at most two such messages $(\echo,-)$ carrying different values. This gives a communication complexity of $O(n^2)$ up to line 5 (c). %(That's how Mostefaoui-Raynal have done it. But what if for a concrete $t_s$ it is $t_s = n/10$ for example, then above argument yields to every honest party echoing 9 messages?) \todo[inline]{This is a good point on the complexity. The complexity should be upper bounded by $O(n^3)$ for any $t_s$, which suffices for our use-case. This will be a problem if we want $O(n^2)$ for some other application, so good to revisit later.}

Next, we show that the communication complexity of $\MV_1$ is bounded by $O(n^3)$. Having a look at Figure \ref{fig:mvbroadcast}, we see that every honest party multicasts at most one message of the form $(\mvii,-)$ (line 4). Furthermore, a message of the form $(\mvi,v)$ for some $v\neq \bot_{mv}$ is multicast if it was received from at least $t_s+1$ distinct parties, ensuring that the message had to come from at least one honest party (line 5). In particular, an honest party only $\mvi$-multicasts at most $n-t_s$ times. Moreover, every honest party multicasts at most one message of the form $(\mvi, \bot_{mv})$ (line 6). As a result, the overall communication complexity of $\MV_1$ is bounded by $O(n^3)$. Getting back to Figure \ref{fig:mvgc}, line 5 (d) and line 6 give two instances of the MV-broadcast protocol with communication complexity $O(n^3)$, so that the overall communication complexity of $\Pi_{\GC}^{t_a, t_s}$ is bounded by $O(n^3)$. 

In the following, we do a communication complexity analysis of $\MV_1$ for the case where the underlying network is asynchronous. Specifically, we show that the communication complexity of $\MV_1$ is bounded by $O(n^2)$ in this case, which leads to an overall complexity of $O(n^2)$ for our graded consensus protocol. We say $\mathit{vote}$ for $v\neq \bot_{rd}$ a message $(\init,v)$ or $(\echo,v)$ sent by some party. Observe that $\MV_1$ is run by an honest party $P_i$ on input $\val$ conditioned on $\output$ being $\true$. In that case, $\val$ is set to either $\bot_{rd}$ or to some $v$ such that $(\msg,v)$ was received by $P_i$ from at least $n-t_s$ distinct parties. We will first show that there are at most five different values $\neq \bot_{rd}$ that are input by the set of honest parties to $\MV_1$. In order for a value $v\neq \bot_{rd}$ to be input to $\MV_1$ by an honest party, $P_i$ must received the message $(\msg,v)$ from at least $n-t_s$ distinct parties. The discussion in the first paragraph tells us that a party can vote for at most three distinct values, while a dishonest party can vote for any number of values. To maximize the total number of values that can be input into $\MV_1$ by the set of honest parties, we consider the worst-case scenario in which there are $t_a$ dishonest parties and if an honest party $P_i$ inputs a value $v$ into $\MV_1$ it has received for this value $n-t_s-t_a$ votes from honest parties and a vote from each of the $t_a$ dishonest parties. Therefore, we have to consider the maximal number of votes that can be sent by the honest parties and the knowledge that only $n-t_s-t_a$ of them are needed to input a value into $\MV_1$. Again by the first paragraph, there are at most $3(n-t_a)$ votes sent by honest parties. It follows that the total number of different values that can be input into $\MV_1$ by the set of honest parties is bounded by the following \begin{align*} \frac{3(n-t_a)}{n-t_s-t_a} = \frac{3(2t_s+1)}{t_s+1} < \frac{6(t_s+1)}{t_s+1} = 6.
\end{align*} As a result, the total number of different values that can be input into $\MV_1$ by the honest parties is bounded by 6 (when including the default value $\bot_{rd}$ also). Now, the same argument as in the previous paragraph applies: a message of the form $(\mvi,v)$ for some $v\neq \bot_{mv}$ is multicast if it was received from at least $t_s+1$ distinct parties, ensuring that the message had to come from at least one honest party and therefore an honest party only $\mvi$-multicasts at most six times (as the previous analysis has shown that there are at most 6 different input values from the set of honest parties). As a consequence, the communication complexity of $\MV_1$ is bounded by $O(n^2)$. Hence, we find that the overall communication complexity of $\Pi_{\GC}^{t_a, t_s}$ is bounded by $O(n^2)$ in case the underlying network is asynchronous. \qed
\end{proof}

\begin{remark}
	From the above analysis it is clear that even in the synchronous case, conditioned on all honest parties having the same input value, the overall communication complexity of the graded consensus protocol is bounded by $O(n^2)$. Again, the reason for this is that in case all honest parties start with the same input value $v\in C$, then an honest party will never echo any other value and as a consequence they all will input $v$ into the $\MV_1$ protocol. On the other hand, when all honest parties input the same value $v$ into $\MV_1$, then by design any honest party will only $\mvii$-multicast that value $v$ and also eventually terminate with it. Having said that, it is clear that the overall communication complexity of $\Pi_{\GC}^{t_a, t_s}$ is bounded by $O(n^2)$ in case the underlying network is synchronous \emph{and} all honest parties start with the same value. This observation is crucial if the graded consensus protocol is used as a building block, as many protocols are build in such a way that the validity property (i.e., all honest parties start with the same value) holds if the underlying network is synchronous. 
\end{remark}


==> mvproof.tex <==
\begin{lemma} 
Let $t_s < n/2$. 
Then $\Pi_{\MV}^{t_a, t_s}$ achieves $t_s$-validity 1. 
\end{lemma} 
\begin{proof} 
Recall that a party $P_i$ only outputs values $v$ such that $|M_2(v)| > 0$ (line 7, Figure \ref{fig:mvbroadcast}).
In order to prove $t_s$-validity 1, we show that no honest party $P_i$ adds a value $v\in V$ to $M_2(v)$ such that $(\mvi,v)$ was multicast only by dishonest parties.
For this, let there be $t_s$ dishonest parties that multicast $(\mvi,v)$ such that $(\mvi,v)$ is not multicast by any honest party.
Since $t_s+1 > t_s$, no honest party echoes the value $v$ and thus $v$ can be received only from the dishonest parties (line 5).
As a consequence, no honest party $P_i$ receives $(\mvi,v)$ from $n-t_s > t_s$ distinct parties and so $M_2(v)$ is never populated by $P_i$ (line 'Updating $M_2(v)$' (i) and (ii)).
\qed
\end{proof} 

\begin{lemma}
Let $t_s < n/2$.
Then $\Pi_{\MV}^{t_a, t_s}$ achieves $t_s$-validity with liveness.
\end{lemma}

\begin{proof}
In order to prove $t_s$-validity with liveness, we show that if every honest party’s input is equal to the same value $v\in V$, then every honest party outputs the set $S = \{v\}$.

Let every honest party multicast $(\mvi,v)$ on the same value $v\in V$ (line 3, Figure \ref{fig:mvbroadcast}).
As argued in the previous proof, no honest party echoes a value $w$ different from $v$ (line 5)
Therefore, at most $t_s$ values different from $v$ are multicast as $(\mvi, -)$ messages.
Now we consider an honest party $P_i$ in the worst case execution, in which the $t_s$ dishonest parties multicast $(\mvi, w)$ on the same value $w\neq v$.
In that case, $|M_1(v)|$ increases monotonically from 0 to $n-t_s$ and $|M_1(w)|$ increases monotonically from 0 to $t_s$.
There are the following two cases.

\sloppy{
\begin{itemize}
\item[(i)] Suppose that $|M_1(w)| \geq |M_1(v)|$.
In this case, the predicate $|\bigcup_{v'\in V} M_1(v')|-|M_1(v_{max})| \geq t_s+1$ in line 6 reduces to $|M_1(v)|\geq t_s+1$ and returns $\false$, since $|M_1(v)|\le |M_1(w)|\le t_s$.
Hence, $P_i$ never multicasts $(\mvi,\bot_{mv})$ (line 6).
\item[(ii)] Suppose that $|M_1(v)| \geq |M_1(w)|$.
In this case, the predicate $|\bigcup_{v'\in V} M_1(v')|-|M_1(v_{max})| \geq t_s+1$ in line 6 reduces to $|M_1(w)|\geq t_s+1$ and returns $\false$, since $|M_1(w)|\le t_s$.
Hence, $P_i$ never multicasts $(\mvi,\bot_{mv})$ (line 6).
\end{itemize}
}
As a result, no honest party multicasts $(\mvi,\bot_{mv})$.
Therefore, no honest party $P_i$ receives $(\mvi,\bot_{mv})$ from $n-t_s > t_s$ distinct parties and $M_2(\bot_{mv})$ is never populated by $P_i$ (line 'Updating $M_2(v)$' (i) and (ii)).
The same is true for the value $w$.
Consequently, every honest party outputs the same set $S = \{v\}$ (line 7).
\qed
\end{proof}

\begin{lemma}
Let $t_s < n/2$. 
Then $\Pi_{\MV}^{t_a, t_s}$ achieves $t_s$-validity 2. 
\end{lemma}

\begin{proof}
This follows directly from $t_s$-validity with liveness.
\qed
\end{proof}

\begin{lemma}
Let $t_a \leq t_s$ and $t_a + 2 \cdot t_s < n$. 
Then $\Pi_{\MV}^{t_a, t_s}$ achieves $t_a$-inclusion. 
\end{lemma}

\begin{proof}
In order to prove $t_a$-inclusion, we show that if honest parties $P_i$ and $P_j$ output sets $S_i$ and $S_j$ respectively, then $S_i = \{w\}$ implies $w\in S_j$ (note that $w = \bot_{mv}$ is possible).

Let honest party $P_i$ output the set $S_i = \{w\}$ (line 7, Figure \ref{fig:mvbroadcast}).
This is conditioned on $|\cup_{v\in V} M_2(v)| \geq n-t_s$ by line 7 and implies that $P_i$ has received $(\mvii,w)$ from at least $n-t_s$ distinct parties by definition of the set $M_2(-)$ in line 'Updating $M_2(v)$' (i) and (ii).
Now consider an honest party $P_j \neq P_i$.
Before $P_j$ outputs the set $S_j$, it has received messages $(\mvii, -)$ from $n-t_s$ distinct parties, that is from at least $n-t_s-t_a > t_s$ honest parties.
Since $(n-t_s)+(t_s+1) > n$, it follows that there is an honest party $P_k$ that sent the same message $(\mvii,v)$ to both $P_i$ and $P_j$.
But since $P_i$ has received only messages $(\mvii,w)$ from $n-t_s$ parties, it follows that $v = w$ and thus $w \in S_j$. 
\qed
\end{proof} 

\begin{lemma}
Let $t_a \leq t_s$ and $t_a + 2 \cdot t_s < n$.
Then $\Pi_{\MV}^{t_a, t_s}$ achieves $t_a$-liveness. 
\end{lemma}

\begin{proof}
In order to prove $t_a$-liveness, we show that every honest party outputs some set.
For this, we first show that every honest party eventually multicasts some $(\mvii, -)$ message (line 4, Figure \ref{fig:mvbroadcast}).
We consider the following predicate $P$: There is a value $v\in V$ such that after some finite time at least $t_s+1$ honest parties have multicast $(\mvi,v)$.
Consider the following two cases.

\begin{itemize}
\item[(i)] The predicate $P$ is satisfied.
In this case, every honest party eventually multicasts $(\mvi,v)$ by construction of $\Pi_{\mathsf{MV}}^{t_a, t_s}$ (line 5).
Since there are at least $n-t_a \geq n-t_s$ honest parties, $\ready$ eventually is set to $\true$ by every honest party due to delivering $(\mvi, v)$ from $n - t_s$ distinct parties (line 4). 
%Therefore, every honest party eventually multicasts some $(\mvii, -)$. 
\item[(ii)] The predicate $P$ is not satisfied.
We consider an honest party $P_i$.
Let $v_{max} = \max_{v' \in V}|M_1(v')$, i.e. the most frequent $\mvi$ value received, and let $r$ be the number of honest parties that multicast $(\mvi,v_{max})$.
Since $P$ is not satisfied, $r \le t_s$.
Since there are at least $n-t_a$ honest parties, $P_i$ receives at least $n-t_a+k$ messages $(\mvi, -)$ with some $k\in [0,t_a]$.
At most $r+k$ of these parties sent message $(\mvi,v_{max})$ to $P_i$, and therefore at least $(n-t_a+k)-(r+k)= n-t_a-r$ of them sent values different from $v_{max}$ to $P_i$.
But since $n-t_a-r \geq n-t_a-t_s > t_s$, the predicate $|\bigcup_{v'\in V} M_1(v')|-|M_1(v_{max})| \geq t_s+1$ in line 6 is satisfied and $P_i$ multicasts $(\mvi,\bot_{mv})$ (line 6).
Analogously, this applies to all honest parties.
And thus, every honest party receives messages $(\mvi,\bot_{mv})$ from at least $n-t_a\geq n-t_s$ distinct parties.
As a result, $\ready$ becomes eventually $\true$ for every honest party (line 4). 
%, and every honest party multicasts some $(\mvii, -)$.
\end{itemize}
This concludes our initial assertion that every honest party eventually multicasts some message $(\mvii,-)$ (by setting $\ready$ to $\true$) by line 4. 

For the final step, we show that every honest party eventually receives \textit{validated} messages $(\mvii, -)$ from at least $n-t_s$ distinct parties and thus outputs a set (namely $\{v : M_2(v) \neq \emptyset \}$) by line 7.
Here, by a \textit{validated} message $(\mvii,w)$ we mean one such that the party has also received messages $(\mvi,w)$ on the same value $w$ from at least $n-t_s$ distinct parties (as is declared in line 4).
By the previous assertion, each honest party $P_i$ multicasts some message $(\mvii, v_i)$ where $v_i$ is such that $|M_1(v_i)| \geq n-t_s$.
Since $(n-t_s)-t_a > t_s$, at least $t_s+1$ honest parties have multicast $(\mvi, v_i)$.
Thus, every honest party eventually multicasts $(\mvi,v_i)$ and for every honest party $P_j$ we have $|M_1(v_i)|\geq n-t_a \geq n-t_s$.
As a consequence, every honest party $P_j$ adds $\{j\}$ to its set $M_2(v_i)$.
Since this proof hitherto also applies to every honest party $P_j$ (in place of $P_i$), eventually every honest party receives validated messages $(\mvii, -)$ from at least $n-t_a\geq n-t_s$ distinct parties and thus outputs the set $\{v : M_2(v) \neq \emptyset \}$ (line 7).
\qed
\end{proof}


==> protocol.tex <==
\section{Main protocol}\label{sec:main_protocol}










\begin{figure}
    \centering
    \includegraphics[width=1.2\textwidth, left]{main_protocol.jpg}
    \caption{Overview of the structure of the main protocol for each party. Beginning with input insertion at the top left with $v_i$, and ending with output production at the bottom left. The values next to arrows indicate the outputs and inputs produced and delivered into procedures.}
    \label{fig:main_protocol}
\end{figure}

































\begin{figure}[ht!] 
\centering
\fbox{
\parbox{0.95\textwidth}{
\centering $\Pi(v_i)$\\
\textbf{Initialization:} $\output_1 = \output_2 = \false$, $T_{\max} = T_1 + T_\sig + T_2 + 1$.
\begin{enumerate}
\item Run $(v_1, g_1) \gets \Pi_{\GCone}(v_i)$. // $T_1$ rounds.
\item Run $v_2 \gets \Pi_\BA^\sig(v_1)$, outputting $v_2 = \bot$ if no output is produced after $T_\sig = O(\kappa)$ rounds, the maximum possible time after each correct party halts with probability $1 - \negl[\kappa]$ given $\adv$ is computationally-bounded.
\item Set $v_3 = v_2$. If $g_1 = 1$: set $v_3 = v_1$.
\item Run $(v_4, g_4) \gets \Pi_\GCtwo(v_3)$. // $T_2$ rounds.
\item Set $\output_1 = \true$.
\item If $g_4 = 1$: multicast $(\decide, v_4)$.
\item At time $T_{\max}$: run $v_\IT \gets \Pi_\BA^\IT(v_4)$, outputting $v_\IT = \bot$ if no output is produced after $T_\IT$ rounds.
\item Set $\output_2 = \true$.
\end{enumerate}
Termination:
\begin{itemize}
\item[C1.] If $\output_1 = \true$ and received $(\decide, v_4)$ from $n - t_s$ distinct parties: output $v_4$ and halt.
\item[C2.] If $\output_2 = \true$ and received for some $v$ $(\decide, v) $ from $n - t_s - t_i$ distinct parties: output $v$ and halt.
\item[C3.] If $\output_2 = \true$: output $v_\IT$ and halt.
\end{itemize}
}
}
\caption{ BA with hybrid security for $2 t_i + t_s < n$ given a $t_s$-secure BA protocol $\Pi_\BA^\sig$, an unconditionally $t_i$-secure BA protocol $\Pi_\BA^\IT$, authenticated $t_s$-secure and $t_i$-valid with termination graded consensus protocol $\Pi_\GCone$ and $t_i$-secure and authenticated $t_s$-valid with termination graded consensus protocol $\Pi_\GCtwo$. \daniel{TODO: add a compiler to make Sig have round gap 1 (maybe can cite something directly)}}
\label{fig:main_protocol}
\end{figure}
\paragraph{Setting $T_\auth$ and $T_\Sab$.} For deterministic protocols, these values should typically be set to $O(t)$ rounds, where the exact value will be protocol-dependent. Randomized protocols $\Pi_\sig^\BA$, such as Katz and Koo's seminal expected constant-round protocol~\cite{C:KatKoo06}, generally provide a guarantee that after each `phase' consisting of a constant number of message delays, honest parties will terminate in this phase or the next with constant probability.
Thus setting $T_\sig = O(\lambda)$ ensures that except with negligible probability, all honest parties terminate.

\paragraph{Information theoretic validity.}
\begin{lemma}
The protocol $\Pi$ is $t_i$-valid.
\end{lemma}
\begin{proof}
By the $t_i$-validity with termination of $\GCone$, all honest parties output $(v, 1)$, where $v$ was input by all honest parties to $\Pi$.
Thereafter, $\Pi_\BA^\sig$ outputs some value, possibly $\bot$, for each party, but since $g_1 = 1$, all honest parties set $v_3 = v$ regardless.
By the $t_i$-security (validity and termination) of $\GCtwo$, all parties output $(v, 1)$ from $\GCtwo$, and so all then multicast $(\decide, v_4)$. Thus all honest parties receive $(\decide, v)$ from $n - t_i \geq n - t_s$ distinct parties, and so all output the same $v$.\daniel{assume $t_i \leq t_s$ somewhere}
\end{proof}

\paragraph{Authenticated validity.}
\begin{lemma}
The protocol $\Pi$ is authenticated $t_s$-valid.
\end{lemma}
\begin{proof}
By the $t_s$-security of $\GCone$, all honest parties output $(v, 1)$ for common honest input $v$.
%Since $v$ is input to $\Pi_\Sig$, by its $t_s$-validity, all honest parties output $v$ given they terminate, which they do with probability $1 - \negl[\kappa]$ by construction of $T_\sig$.
Then as above, since all honest parties output $g_1 = 1$, all honest parties set $v_3 = v$.
By the $t_s$-validity with termination of $\GCtwo$, all parties output $(v, 1)$.
Validity then follows as in the proof of Lemma~\ref{lemma:main_no_sig_validity}
\end{proof}

\paragraph{Information theoretic consistency.}
\begin{lemma}\label{lemma:main_no_sig_consistency}
The protocol $\Pi$ is $t_i$-consistent.
\end{lemma}
\begin{proof}
Suppose that at least one honest party outputs due to C1, i.e., receives $(\decide, v_4)$ from $n - t_s$ distinct parties.
Since $n - t_s - t_i > t_i + 1$, at least one honest party must have output $(v_4, 1)$ from $\GCtwo$, and thus by $t_i$-consistency of $\GCtwo$, all honest parties output the same value $v_4$, and in particular no honest party multicasts $(\decide, v_4')$ for $v_4' \neq v_4$.
In addition, at least $n - t_s - t_i$ honest parties must have multicast $(\decide, v_4)$.
%Then at least $n - t_s - t_i$ honest parties multicast $(\decide, v_4)$ since $g_4 = 1$.
Thus all honest parties will receive $(\decide, v_4)$ from at least $n - t_s - t_i$ distinct parties, and not for any other value $v_4' \neq v_4$ since $n - t_s - t_i > t_i$.
Therefore all honest parties will output $v_4$ either due to C1 or C2.

Suppose that no honest party outputs due to C1 and at least one outputs due to C2, i.e., due to receiving $(\decide, v)$ for some $v$ from $n - t_s - t_i$ distinct parties.
Then at least one honest party must have multicast $(\decide, v)$, since $n - t_s - t_i > t_i$.
By the $t_i$-consistency of $\GCtwo$, all honest parties will propose the same $v$ to $\Pi_\IT$.
By the $t_i$-validity of $\Pi_\BA^\IT$, all honest parties will output the same $v_\IT = v$.
Thus all honest parties will output either due to C2 or C3 with the same value $v$.

Finally, supposing no honest party outputs due to C1 or C2, all honest parties output the same value $v$ from $\Pi_\BA^\IT$ due to the $t_i$-consistency of $\Pi_\BA^\IT$ and then decide it due to C3.
\end{proof}

\paragraph{Authenticated consistency.}
\begin{lemma}\label{lemma:main_sig_consistency}
The protocol $\Pi$ is authenticated $t_s$-consistent.
\end{lemma}
\begin{proof}
We first argue that all honest parties input the same value $v_3$ to $\Pi_\GCtwo$. 
\begin{itemize}
    \item Suppose first that at least one honest party outputs $g_1 = 1$ from $\Pi_\GCone$. Then by the $t_s$-consistency of $\Pi_\GCone$, all honest parties will output the same $v_1$. By the $t_s$-validity of $\Pi_\IT$, all honest parties output $v_2 = v_1$ from $\Pi_\BA^\sig$. Thus $v_3$ is the same for all honest parties.
    \item Otherwise, no party outputs $g_1 = 1$ from $\Pi_\GCone$. By $t_s$-consistency of $\Pi_\BA^\sig$, all honest parties output the same $v_2$, and by construction all set $v_3 = v_2$ (i.e., do not override $v_3$ with $v_1$).
\end{itemize}
Then, by the $t_s$-validity with termination of $\GCtwo$, all honest parties output $(v_4, 1)$ from $\Pi$, multicast $(\decide, v_4)$, and by the same reasoning as for the proof of Lemma~\ref{lemma:main_sig_validity}, all honest parties will output due to C1 (and in particular never execute $\Pi_\BA^\IT$).
\end{proof}

\paragraph{Liveness and termination.}
\begin{lemma}\label{lemma:main_liveness}
The protocol $\Pi$ satisfies authenticated $t_s$-liveness and authenticated $t_s$-termination, as well as $t_i$-liveness and $t_i$-termination.
\end{lemma}
\begin{proof}
We begin with $t_s$-liveness and termination.
By the $t_s$-security of $\GCone$ and $\Pi_\BA^\sig$, both protocols terminate ($\GCone$ in $T_1$ rounds and $\Pi_\BA^\sig$ with probability $1 - \negl[\kappa]$ by construction.
By the $t_s$-validity with termination of $\GCtwo$, $\GCtwo$ outputs in $T_2$ rounds.
By the same argument as for $t_s$-consistency (Lemma~\ref{lemma:main_sig_consistency}), all honest parties output and halt due to C1.
A similar argument holds for $t_i$-security, except using the $t_i$-validity and termination of $\GCone$, $t_s$-security of $\GCtwo$ and $t_i$-security of $\Pi_\BA^\IT$.
\end{proof}


==> rr.tex <==
\def\RR{\mathsf{RR}}
\def\PKI{\mathsf{PKI}}
\def\Sig{\mathsf{Sig}}
\def\Auth{\mathsf{Auth}}

\section{Signature-Based Byzantine Agreement with Proof-of-Work Fallback}
Consider a computationally-bounded adversary that can corrupt at most $t < n/2$ parties.
Suppose that at least one of the following assumptions hold:
\begin{enumerate}
\item A consistent PKI is available to all honest parties. 
\item All parties can make at most $q$ queries to hash function $H$ each round (modelling $H$ as a random oracle). 
\end{enumerate}
Note in the latter case that we do \emph{not} assume any setup -- it is well known that without setup or restrictions on the adversary that $t < n/3$ is optimal to solve consensus.
It was shown recently by Garay et al.~\cite{EC:GKOPZ20} that consensus is in fact possible (and optimal) in this resource-restricted setting given $t < n/2$.
In this section, we construct a resilience-optimal protocol that is secure if at least one of the above assumptions holds.
\subsection{Protocol}
See Figure~\ref{fig:rrhybrid}.
\begin{figure}[ht!] 
\centering
\fbox{
\parbox{0.95\textwidth}{
\centering $\Pi_{\BA}^{\Auth \lor \RR}(v_i)$
\begin{enumerate}
\item Run $\vec{\pk} \gets \Pi_\PKI^\RR$
\item Run $v \gets \texttt{Compile}(\Pi_{\BA}^\Auth, \vec{\pk})$
\item Output $v$ and terminate.
\end{enumerate}
Compiler $\texttt{Compile}(\Pi_{\sig}, \vec{\pk})$:
\begin{itemize}
\item If TS, first run DKG/setup protocol for TS keys using $\vec{\pk}$ (probably not worth it though for single-shot)
\item Replace sign/ts sign calls with two sign/ts sign calls.
\item Replace verify/ts verify calls with two verify/ts verify calls.
\end{itemize}
}
}
\caption{$t$-secure assumption-agnostic synchronous consensus $\Pi_\BA^{\Auth \lor \RR}$ with $t < n/2$ given a resource-restricted PKI establishment protocol $\Pi_{\PKI}^\RR$ and an authenticated consensus protocol $\Pi_{\BA}^\Auth$.}
\label{fig:rrhybrid}
\end{figure}
\subsection{Proof}
Reduce to the security of the original protocol/the setup; very simple.
\subsection{Remarks}
\begin{itemize}
\item Optimal from Fitzi (honest majority is needed for BA);
\item Can use e.g. BLS signatures to keep the same communication complexity for signatures in $\Pi_\BA^\Auth$ rather than the naive $2\kappa$ by using 2 schemes in parallel (what about for threshold sigs?)
\item Can re-use PKI/setup over many runs with some care.
\item Instantiation of $\Pi_\PKI^\RR$: Can use \cite{EC:GKOPZ20} (linear rounds, poly CC); can plausibly do $O(\kappa)$ rounds by adapting \cite{PKC:GKLP18} (which gives a pseudonymous PKI, i.e. possibly more than 1 key per honest party, but keys controlled y an honest majority of parties). To formalize? Can we improve CC?
\item Works with our information-theoretic compiler as well.
\end{itemize}
